Including Facial Expressions in Contextual Embeddings for Sign Language Generation

State-of-the-art sign language generation frameworks lack expressivity and naturalness which is the result of only focusing manual signs, neglecting the affective, grammatical and semantic functions of facial expressions. The purpose of this work is to augment semantic representation of sign language through grounding facial expressions. We study the effect of modeling the relationship between text, gloss, and facial expressions on the performance of the sign generation systems. In particular, we propose a Dual Encoder Transformer able to generate manual signs as well as facial expressions by capturing the similarities and differences found in text and sign gloss annotation. We take into consideration the role of facial muscle activity to express intensities of manual signs by being the first to employ facial action units in sign language generation. We perform a series of experiments showing that our proposed model improves the quality of automatically generated sign language.

==> sections/related_work.tex <==
\section{Related Work}



==> sections/results_tables.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|ccccc|ccccc}
\toprule
 \multirow{2}{*}{\textbf{Components}} & \multicolumn{5}{c|}{\textbf{Dev Set}} &  \multicolumn{5}{c}{\textbf{Test Set}} \\
& \multicolumn{1}{c}{Bleu$_1$} & \multicolumn{1}{c}{Bleu$_2$} & \multicolumn{1}{c}{Bleu$_3$} & \multicolumn{1}{c}{Bleu$_4$} & \multicolumn{1}{c|}{ROUGE} & \multicolumn{1}{c}{Bleu$_1$} & \multicolumn{1}{c}{Bleu$_2$} & \multicolumn{1}{c}{Bleu$_3$} & \multicolumn{1}{c}{Bleu$_4$} & \multicolumn{1}{c}{ROUGE} \\ 
\cmidrule[1pt]{2-11}
\begin{tabular}[c]{@{}c@{}}Manual\end{tabular} & 30.15 & 20.58 & 15.41 & 12.22 & 30.41 & 27.76 & 18.86 & 14.11 & 11.32 & 27.44 \\
%\midrule
%\begin{tabular}[c]{@{}c@{}}Hands \& Body + 2D Face \end{tabular} & 27.29 & 18.24 & 13.62 & 10.71 & 27.26 & 26.35 & 17.38 & 12.92 & 10.39 & 25.60\\
%\midrule
\begin{tabular}[c]{@{}c@{}}Manual and Facial\end{tabular} & 29.46 & 20.30 & 15.31 & 12.10 & 29.25 & 26.75 & 17.88 & 13.29 & 10.61 & 26.54\\
%\midrule
%\begin{tabular}[c]{@{}l@{}}Hands \& Body + 3D Face\end{tabular} & 27.54 & 18.58 & 13.77 & 10.87 & 27.90 & 27.00 & 18.23 & 13.63 & 10.89 & 26.89 \\
%\midrule
%\begin{tabular}[c]{@{}l@{}}Hands \& Body + 3D Face \\ + Facial AU\end{tabular} & 26.70 & 18.00 & 13.37 & 10.64 & 27.02 & 24.67 & 16.45 & 12.14 & 9.73 & 25.03 \\
\bottomrule
\end{tabular}
\caption{Translation results of the SLT model~\cite{camgoz2020sign} used for backtranslation when trained and evaluated with ground truth hand and body skeleton joints (manual) and facial landmarks and AUs (facial).}
\label{tab:slt}
\end{table*}


\begin{table*}[!ht]
\centering
\begin{tabular}{c|ccccc|ccccc}
\toprule
 \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Dev Set}} &  \multicolumn{5}{c}{\textbf{Test Set}} \\
& \multicolumn{1}{c}{Bleu$_1$} & \multicolumn{1}{c}{Bleu$_2$} & \multicolumn{1}{c}{Bleu$_3$} & \multicolumn{1}{c}{Bleu$_4$} & \multicolumn{1}{c|}{ROUGE} & \multicolumn{1}{c}{Bleu$_1$} & \multicolumn{1}{c}{Bleu$_2$} & \multicolumn{1}{c}{Bleu$_3$} & \multicolumn{1}{c}{Bleu$_4$} & \multicolumn{1}{c}{ROUGE} \\ 
\cmidrule[1pt]{2-11}
G2S  & 24.51 & 15.71 & 11.19 & 8.70 & \textbf{24.84} & \textbf{23.26} & 14.54 & 10.21 & 7.84 & 22.89\\
T2S  & 22.90 & 14.55 & 10.42 & 8.14 & 23.42 & 22.14 & 13.88 & 9.85 & 7.56 & 22.50\\
TG2S (Ours) & \textbf{24.60} & \textbf{16.20} & \textbf{11.68} & \textbf{8.97} & 24.82 & 22.97 & \textbf{14.71} & \textbf{10.59} & \textbf{8.19} & \textbf{23.45}\\
\bottomrule
\end{tabular}
\caption{Back translation results obtained from the generative models when using only manual features. Our proposed model has the highest scores in almost all metrics compared to the models using only gloss or text.}
\label{tab:handsbody}
\end{table*}

% \begin{comment}
% \begin{table*}[]
% \centering
% \begin{tabular}{c|ccccc|ccccc}
% \toprule
%  \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Dev Set}} &  \multicolumn{5}{c}{\textbf{Test Set}} \\
% & \multicolumn{1}{c}{Bleu$_1$} & \multicolumn{1}{c}{Bleu$_2$} & \multicolumn{1}{c}{Bleu$_3$} & \multicolumn{1}{c}{Bleu$_4$} & \multicolumn{1}{c|}{ROUGE} & \multicolumn{1}{c}{Bleu$_1$} & \multicolumn{1}{c}{Bleu$_2$} & \multicolumn{1}{c}{Bleu$_3$} & \multicolumn{1}{c}{Bleu$_4$} & \multicolumn{1}{c}{ROUGE} \\ 
% \cmidrule[1pt]{2-11}
% G2S            & {[}22.74, 22.65{]}             & {[}14.92,15.08{]}              & {[}10.99,10.98{]}              & {[}8.58,8.56{]}                & {[}23.91, 23.67{]}            \\
% T2S            & {[}16.54/20.86{]}              & {[}9.72/13.14{]}               & {[}6.78/9.49{]}                & {[}5.18/7.45{]}                & {[}18.80/22.50{]}             \\
% TG2S           & {[}21.92/21.22{]}              & {[}13.49/13.51{]}              & {[}9.41/9.68{]}                & {[}7.06/7.51{]}                & {[}22.77/22.10{]}            
% \end{tabular}
% \label{tab:facial}
% \caption{Backtranslation results when using hand and body skeleton joints as well as facial landmarks.}
% \end{table*}
% \end{comment}

\begin{table*}[]
\centering
\begin{tabular}{c|ccccc|ccccc}
\toprule
 \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{Dev Set}} &  \multicolumn{5}{c}{\textbf{Test Set}} \\
& \multicolumn{1}{c}{Bleu$_1$} & \multicolumn{1}{c}{Bleu$_2$} & \multicolumn{1}{c}{Bleu$_3$} & \multicolumn{1}{c}{Bleu$_4$} & \multicolumn{1}{c|}{ROUGE} & \multicolumn{1}{c}{Bleu$_1$} & \multicolumn{1}{c}{Bleu$_2$} & \multicolumn{1}{c}{Bleu$_3$} & \multicolumn{1}{c}{Bleu$_4$} & \multicolumn{1}{c}{ROUGE} \\ 
\cmidrule[1pt]{2-11}
G2S & 16.11 & 8.77 & 5.97 & 4.49 & 16.19 & 16.29 & 9.20 & 6.37 & 4.93 & 16.73\\
T2S & 15.65 & 8.35 & 5.76 & 4.44 & 15.65 & 14.12 & 7.76 & 5.53 & 4.39 & 14.82\\
TG2S & \textbf{17.25} & \textbf{10.17} & \textbf{7.04} & \textbf{5.32} & \textbf{17.85} & \textbf{17.18} & \textbf{10.39} & \textbf{7.39} & \textbf{5.76} & \textbf{17.64}\\
\bottomrule
\end{tabular}
\caption{Back translation results obtained from the generative models when using manual features and facial landmarks and AUs. Our proposed model has the highest scores in all metrics compared to the models using only gloss or text. }
\label{tab:auc}
\end{table*}

==> todo.tex <==
1) Another weakness of the paper is its writing. There are typos and long unclear sentences in the paper. This could be alleviated by breaking some of these long sentences or using better punctuation.

Done 2)Fix: "The purpose of this work is to improve sign language generation by modeling the relationship of text which is rich in adjectives and gloss which represents manual signs but lacks information on ad- jectives represented by facial expressions."

Done 3)Fix:"written spoken languages"?

Done 4)Fix: "sym- bolic representations" -> symbolic

Done 5)Proposed architecture decisions might need more reasoning. For example: "As the N ̸= U , we stack hn vertically for U times and stack hu vertically for N times in order to have two matrices with the same dimensions. Then we multiply both matrices with the Hadamard multiplication."

6)Describe more about the evaluation: "is there another way to evaluate your results? Using Blue score might not be the best way for evaluating these type of results; and by using another metric you could actually show the advantage of using your approach"

7)Explain more: The results presented in Tables 2-4 are very low, especially the BLEU score. It would be important to discuss what are realistic results for this task and upper ceiling, as well as to discuss the potential issues that may arise from such low results if the system is used in a pilot study. Due to very low results reported in Tables 2-4, it would be important to discuss in more details failure modes of the system, e.g. are there some particular constructions or topics the system fails at, are their some ethical implications of the system's failures?

Done 8)Give details of the statistical test: What was the statistical significance test used for Table 1? When reporting p<0.05, it is also important to know if the right test of statistical significance was used.

Done 9)Statistical significance explanation again: Are the differences between the results of various systems in Tables 2-4 statistically significant? Numerically, some of them are very close. Therefore, it is necessary to report statistical significance of the differences, e.g. by using random sampling techniques on the test set.

Done 10)Fix typo: Grammatical Facial Expressions: "the upper example"rain"" -> a space is missing

Done 11) Fix typo:  Sign Language Generation: "2020).(Saunders, Camgoz, and Bowden 2021) are the first to..." -> a space is missing after "."; it should be "Saunders, Camgoz, and Bowden (2021) are first to..."

Maybe not necessary 12) Figures 4 and 5 could be moved to an appendix to allow for the necessary discussion and more thorough error analysis.

13)The results in Tables 3 and 4 seem to be unfair because the inputs of G2S/T2S/TG2S are not the same. Besides, the results of G2S/T2S are different from the ones published in [R1]. More details and explanation should be provided.

Done 14)Several important references are missing, such as [R2] [R3]. 
[R2] Mixed SIGNals: Sign Language Production via a Mixture of Motion Primitives, ICCV 2021. 
[R3] Adversarial Training for Multi-Channel Sign Language Production, BMVC 2020.

Not including 15) Figure 4 only shows the performance of this work on word-level sign language generation. What is the visualization effect on sentence-level sign language generation?

16) Explain: What is the Back Translation model (BT model) used in this paper? Can you provide more details about processing the generated pose into input to the BT model?

Done 17)Paraphrase the Title to: Augmenting Semantic representation of sign language through grounding/including facial expressions.

18) The reviewer would prefer some details about the evaluation approach that the authors used. What the reviewer understands is the input to the model is text and gloss and output is facial AU and landmarks that produce the sign. When evaluating between original text and text generated from Sign Language Transformer using BLEU and
ROUGE, do the text generation model uses the sign produced from the proposed model? It will be helpful to explain or perhaps add a diagram outlining this.

Future Work 19)Considering the impact of the problem, a more comprehensive evaluation technique would be a user study with real sign language users. Since the authors do not mention this in the future plan, the reviewer suggests evaluation with a user study and other datasets.

20)Typo: The paper needs a thorough grammar check. There are several cases of typos and incomplete sentences (e.g. on the other, hand, In addition facial expressions, etc.)

Done 21)Intro: When you look at gloss system, if you completely exclude facial expression then the meaning is lost. We are including facial action unit analysis and augment how  we can learn semantic spaces or representations for sign language. We test our hypothesis by doing backtranslation.

Done 22)Check the author response that malihe sent



